Classification of charge-conserving loop braid representations

Here a loop braid representation is a monoidal functor $\mathsf{F}$ from the loop braid category $\mathsf{L}$ to a suitable target category, and is $N$-charge-conserving if that target is the category $\mathsf{Match}^N$ of charge-conserving matrices (specifically $\mathsf{Match}^N$ is the same rank-$N$ charge-conserving monoidal subcategory of the monoidal category $\mathsf{Mat}$ used to classify braid representations in arXiv:2112.04533) with $\mathsf{F}$ strict, and surjective on $\mathbb{N}$, the object monoid. We classify and construct all such representations. In particular we prove that representations fall into varieties indexed by a set in bijection with the set of pairs of plane partitions of total degree $N$.

==> macros-tetra.tex <==

%% some argy-bargy about the notation for level. let's adopt
%\newcommand{\NL}{N}  %% for now.



%{{{ TRI and TETRA MACROS

\newcommand{\fii}{\mathsf{f}} %% ferro
\newcommand{\ai}{\mathsf{a}}  %% antoferro
%\newcommand{\pfii}{\overline{f}} %% +_f
\newcommand{\pfii}{{\fii}} %% +_f
\newcommand{\uppfii}{\pfii}
%\newcommand{\pai}{\overline{a}}
\newcommand{\pai}{{\ai}}
\newcommand{\mfii}{\underline{\fii}} %% -_f
\newcommand{\mai}{\underline{\ai}}
\newcommand{\uppai}{\pai}
%\newcommand{\ooo}[1]{\textcircled{\tiny #1}}
\newcommand{\ooo}[1]{\textcolor{orange}{\textcircled{\tiny #1}}}

\newcommand{\ber}[5]{ %% draws a triangle rep of \alpha(F(\sigma))
%% here $a_1$ is hard-wired.
\xymatrix{
%       &  {a_{#1}}_{\ooo{2}} \ar[dr]^{#4} \\
%{{a_1}}^{\ooo{1}} \ar[ur]^{#3} \ar[rr]^{#5} &&  {}_{\ooo{3}}{a_{#2}}
       &  {a_{#1}}_{\ooo{2}} \ar[dr]|{#4} \\
{{a_1}}^{\ooo{1}} \ar[ur]|{#3} \ar[rr]|{#5} &&  {}_{\ooo{3}}{a_{#2}}
}}

\newcommand{\berm}[6]{ %% draws a triangle rep of \alpha(F(\sigma))
\xymatrix{
       &  {a_{#2}}_{\ooo{2}} \ar[dr]^{#5} \\
{{a_{#1}}}^{\ooo{1}} \ar[ur]^{#4} \ar[rr]^{#6} &&  {}_{\ooo{3}}{a_{#3}}
}}

\newcommand{\bermss}[6]{ %% draws a triangle rep of \alpha(F(\sigma))
%% here two edges are identified
\xymatrix{
%       &  {a_{#2}}_{\ooo{2}} \ar[dr]^{#5}_{}="b" \\
       &  {a_{#2}}_{\ooo{2}} \ar[dr]|{#5}="b" \\
%{{a_{#1}}}^{\ooo{1}} \ar[ur]^{#4}_{}="a" \ar[rr]^{#6} &&  {}_{\ooo{3}}{a_{#3}}
%\ar@{=}_{} "a";"b"
{{a_{#1}}}^{\ooo{1}} \ar[ur]|{#4}="a" \ar[rr]|{#6} &&  {}_{\ooo{3}}{a_{#3}}
\ar@{=}_{} "a";"b"
}}

\newcommand{\bermpp}[6]{ %% draws a triangle rep of \alpha(F(\sigma))
%% here all edges are identified
\xymatrix{
%       &  {a_{#2}}_{\ooo{2}} \ar[dr]^{#5}_{}="b" \\
       &  {a_{#2}}_{\ooo{2}} \ar[dr]|{#5}="b" \\
%{{a_{#1}}}^{\ooo{1}} \ar[ur]^{#4}_{}="a" \ar[rr]^{#6}="c" &&  {}_{\ooo{3}}{a_{#3}}
{{a_{#1}}}^{\ooo{1}} \ar[ur]|{#4}="a" \ar[rr]|{#6}="c" &&  {}_{\ooo{3}}{a_{#3}}
\ar@{=}_{} "a";"b"
\ar@{=}_{} "a";"c"
\ar@{=}_{} "b";"c"
}}

\newcommand{\mbermpp}[9]{ %% draws a triangle rep of \alpha(F(\sigma))
%% here all edges are identified
%       &  {a_{#2}}_{\ooo{2}} \ar[dr]^{#5}_{}="b" \\
       &  {a_{#2}}_{\ooo{2}} \ar[dr]|{#5}="b" \\
%{{a_{#1}}}^{\ooo{1}} \ar[ur]^{#4}_{}="a" \ar[rr]^{#6}="c" &&  {}_{\ooo{3}}{a_{#3}}
{{a_{#1}}}^{\ooo{1}} \ar[ur]|{#4}="a" \ar[rr]|{#6}="c" &&  {}_{\ooo{3}}{a_{#3}}
\ar@{=}|{#7} "a";"b"
\ar@{=}|{#8} "a";"c"
\ar@{=}|{#9} "b";"c"
}

\newcommand{\mbermupp}[9]{ %% draws a triangle rep of \alpha(F(\sigma))
%% here all edges are identified
%       &  {{#2}}_{\ooo{2}} \ar[dr]^{#5}_{}="b" \\
       &  {{#2}}_{\ooo{2}} \ar[dr]|{#5}="b" \\
%{{a_{#1}}}^{\ooo{1}} \ar[ur]^{#4}_{}="a" \ar[rr]^{#6}="c" &&  {}_{\ooo{3}}{a_{#3}}
{{{#1}}}^{\ooo{1}} \ar[ur]|{#4}="a" \ar[rr]|{#6}="c" &&  {}_{\ooo{3}}{{#3}}
\ar@{=}|{#7} "a";"b"
\ar@{=}|{#8} "a";"c"
\ar@{=}|{#9} "b";"c"
}

\newcommand{\abcab}{\ar@{=}_{} "a";"b"}
\newcommand{\abcac}{\ar@{=}_{} "a";"c"}
\newcommand{\abcbc}{\ar@{=}_{} "b";"c"}

\newcommand{\bermxx}[7]{ %% draws a triangle rep of \alpha(F(\sigma))
%% here some edges are identified as per #7
\xymatrix{
%       &  {a_{#2}}_{\ooo{2}} \ar[dr]^{#5}_{}="b" \\
%{{a_{#1}}}^{\ooo{1}} \ar[ur]^{#4}_{}="a" \ar[rr]^{#6}="c" &&  {}_{\ooo{3}}{a_{#3}}
%#7
       &  {a_{#2}}_{\ooo{2}} \ar[dr]|{#5}="b" \\
{{a_{#1}}}^{\ooo{1}} \ar[ur]|{#4}="a" \ar[rr]|{#6}="c" &&  {}_{\ooo{3}}{a_{#3}}
#7
%\ar@{=}_{} "a";"b"
%\ar@{=}_{} "a";"c"
%\ar@{=}_{} "b";"c"
}}

%}}}
%{{{ TETRA MACROS

\newcommand{\Mercedes}{dragon-eye}

\newcommand{\bertx}[9]{  %% an older verion of \bert
\xymatrix@R=37pt{
& {}^{a_{#1}} \ooo{2}_{} \ar[rr]^{#5} \ar[drrr]^{#8}  && \ooo{3}^{a_{#2}} \ar[dr]^{#7} \\
{}_{a_1}\ooo{1} \ar[ur]^{#4} \ar[urrr]^{#6} \ar[rrrr]^{#9} &&&& \ooo{4}_{a_{#3}}
}}

\newcommand{\bert}[9]{ %% a tetra rep of \alpha(F(\sigma))
\xymatrix@R=37pt{
& {a_{#1}}_{\ooo{2}} \ar[rr]^{#5} \ar[drrr]^{#8}  && {}_{\ooo{3}}{a_{#2}} \ar[dr]^{#7} \\
{{a_1}}^{\ooo{1}} \ar[ur]^{#4} \ar[urrr]^{#6} \ar[rrrr]^{#9} &&&& {}^{\ooo{4}}{a_{#3}}
}}

\newcommand{\berto}[9]{ %% tetra rep that is planar
\xymatrix@C=10pt{
1 \ar[drr]^{#4}="a"
  \ar@/^1pc/@{=}[rrrrrr]
           &&                  &          &
                                           && 1
                                           \ar[dll]^{#5}_{\;\;\;}="b"
                                           \ar@/^2pc/@{=}[dddlll] \\
           && #1 \ar[rr]^{#6}="c" \ar[dr]^{#7} &          & #3   \\
           &&                  & #2 \ar[ur]^{#8} &   \\
           &&                  & 1 \ar[u]^{#9} \ar@/^2pc/@{=}[uuulll]
%           \ar@{=} "a";"b"
%            \ar@{=} "b";"c"
%            \ar@{=} "a";"c"
}}

\newcommand{\bertovold}[9]{ %% tetra rep that is planar
\xymatrix@C=10pt{
1 \ar[drr]^{#4}="a"
  \ar@/^1pc/@{=}[rrrrrr]
           &&                  &          &
                                           && 1
                                           \ar[dll]^{#5}_{\;\;\;}="b"
                                           \ar@/^2pc/@{=}[dddlll] \\
           && #1 \ar[rr]^{#6}="c" \ar[dr]_{#7} &          & #3   \\
           &&                  & #2 \ar[ur]^{#8} &   \\
           &&                  & 1 \ar[u]^{#9} \ar@/^2pc/@{=}[uuulll]
           \ar@{=} "a";"b"
            \ar@{=} "b";"c"
            \ar@{=} "a";"c"
}}

\newcommand{\bertov}[9]{ %% tetra rep that is planar
\xymatrix@C=10pt{
1 \ar[drr]|{#4}="a"
  \ar@/^1pc/@{=}[rrrrrr]
           &&                  &          &
                                           && 1
                                           \ar[dll]|{#5}="b"
                                           \ar@/^2pc/@{=}[dddlll] \\
           && #1 \ar[rr]|{#6}="c" \ar[dr]|{#7} &          & #3   \\
           &&                  & #2 \ar[ur]|{#8} &   \\
           &&                  & 1 \ar[u]|{#9} \ar@/^2pc/@{=}[uuulll]
           \ar@{=} "a";"b"
            \ar@{=} "b";"c"
            \ar@{=} "a";"c"
}}

\newcommand{\abcccc}{ %% identifying edge matrices
        \ar@{=} "a";"b"
        \ar@{=} "b";"c"
        \ar@{=} "a";"c"    }

\newcommand{\cdeeee}{ %% identifying edge matrices
        \ar@{=} "c";"d"
        \ar@{=} "d";"e"
        \ar@{=} "c";"e"    }

\newcommand{\adffff}{ %% identifying edge matrices
        \ar@/_/@{=} "a";"d"
        \ar@/_/@{=} "d";"f"
        \ar@/_/@{=} "a";"f"    }

\newcommand{\beffff}{ %% identifying edge matrices
        \ar@/^/@{=} "b";"e"
        \ar@/^/@{=} "e";"f"
        \ar@/^/@{=} "b";"f"    }

\newcommand{\bertoxx}[9]{ %% tetra rep that is planar (takes idents as
%% final argument).
\xymatrix@C=10pt{
1 \ar[drr]|{#4}="a"
  \ar@/^1pc/@{=}[rrrrrr]
           &&                  &          &
                                           && 1
                                           \ar[dll]^{#5}_{\;\;\;}="b"
                                           \ar@/^2pc/@{=}[dddlll] \\
           && #1 \ar[rr]|{#6}="c" \ar[dr]_{#7} &          & #3   \\
           &&                  & #2 \ar[ur]_{#8} &   \\
           &&                  & 1 \ar[u]^{9} \ar@/^2pc/@{=}[uuulll]
#9
%           \ar@{=} "a";"b"
%            \ar@{=} "b";"c"
%            \ar@{=} "a";"c"
}}

\newcommand{\bertox}[9]{ %% tetra rep that is planar (takes idents as
%% final argument).
\xymatrix@C=10pt{
1 \ar[drr]|{#4}="a"
  \ar@/^1pc/@{=}[rrrrrr]
           &&                  &          &
                                           && 1
                                           \ar[dll]|{#5}="b"
                                           \ar@/^2pc/@{=}[dddlll] \\
           && #1 \ar[rr]|{#6}="c" \ar[dr]|{#7}="d" &          & #3   \\
           &&                  & #2 \ar[ur]|{#8}="e" &   \\
           &&                  & 1 \ar[u]|{\x}="f" \ar@/^2pc/@{=}[uuulll]
#9
%           \ar@{=} "a";"b"
%            \ar@{=} "b";"c"
%            \ar@{=} "a";"c"
}}

\newcommand{\pyr}[9]{
\xymatrix@C=30pt@R=13pt{
1 \ar[rr]|{#1} \ar[dr]|{#2} \ar[dddr]|{#3}
                         &                  & #9 \\
                         & #7 \ar[ur]|{#4} \ar[dd]|{#5}    \\ \\
                         & #8 \ar[uuur]|{#6}
}}

%}}}


\newcommand{\qquadd}{\hspace{.21cm} & \hspace{.21in}}

%{{{ macros etc and upp upp upp

\newcommand{\alp}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\lemx}{the X~Lemma}
\newcommand{\loone}{\mat{cc} \!\alp\!+\!\be & -\alp\be\! \\ 1&0\tam  }
\newcommand{\ccc}{\bullet}
%%% next is a triangle
\newcommand{\trin}[6]{ \xymatrix{& #3\; \ccc\;\; \ar@{-}[dr]^{#4}
\\
#1 \ccc \ar@{-}[rr]_{#6} \ar@{-}[ur]^{#2} && \ccc #5  }}



%}}}




==> macros/macros.tex <==

\newcommand{\todocd}[1]{{\textcolor{magenta}{#1}}}
\newcommand{\todopm}[1]{{\textcolor{blue}{#1}}}
\newcommand{\ppm}[1]{{\textcolor{red}{#1}}}
\newcommand{\ppmm}[1]{{\textcolor{brown}{#1}}}
\newcommand{\ppmx}[1]{}
\newcommand{\todoer}[1]{{\textcolor{orange}{#1}}}


% environments 
%------------------------------------------------------------------------------------

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}



\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{question}[theorem]{Question}
\newtheorem{claim}[theorem]{Claim}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}



% definitions  
%------------------------------------------------------------------------------------

\newcommand{\beq}{\begin{equation}}
\newcommand{\eq}{\end{equation}} 
\newcommand{\mat}{\left( \begin{array}}
\newcommand{\tam}{\end{array} \right)} 

\newcommand{\ignore}[1]{}  
%\newcommand{\ul}[1]{\underline{#1}}  %% in macros2


\newcommand\Nn{\mathbb{N}}
\newcommand\Zz{\mathbb{Z}}
\newcommand\Qq{\mathbb{Q}}
\newcommand\Rr{\mathbb{R}}
\newcommand\Cc{\mathbb{C}}
\newcommand{\C}{\mathbb{C}}

\newcommand\BB[1]{B_{#1}}	% braid groups
\newcommand{\B}{B}              % braid group hook v.2.0!
\newcommand{\rhob}{{\mathbf \varrho}}  % hook for Burau rep
\newcommand \ep{\varepsilon}
\newcommand{\Sym}{\Sigma}        % symmetric group
\newcommand{\SymXZ}{\Zz_2\times\Sigma}        % Z x symmetric group
%\newcommand{\GG}{{\mathcal G}}    %% in macros2  \GG is \Sym x Z_2

\newcommand \F[1]{F_{#1}} % free groups

\newcommand\id{\mathrm{id}} % identity 
\newcommand\ie{{\textit{i.e.}}} % e.g.
\newcommand\ii{i}
\newcommand\inv{^{-1}} % inverse 
\newcommand\jj{j}

\newcommand\LB[1]{LB_{#1}}	% loop braid groups
\newcommand\LH{L\!H}	% loop Hecke
\newcommand{\HLB}{LH}  %% conforming the main algebra name (not!)
\newcommand{\LBcat}{{\mathsf{ LB}}}  %% a cat hook
\newcommand{\Bcat}{{\mathsf{ B}}}    %% a cat hook
\newcommand{\Hcat}{{\mathsf{ H}}}    %% a cat hook
%\newcommand{\LHcat}{{\mathsf{ LH}}}  %% a cat hook
\newcommand{\LHcat}{{{LH}}}  %% a cat hook
\newcommand{\Mat}{{\mathsf{ Mat}}}   %% a cat hook
\newcommand{\Vect}{{\mathsf{ Vect}}} %% a cat hook
\newcommand{\ann}{Ann\,}
\newcommand{\fb}[1]{\framebox{#1}} % framebox for matrix substructures
\newcommand{\SPe}{S\!P}
\newcommand{\Gx}{G_{\chi}} % functor
\newcommand{\func}[2]{#1-\!\!\!\!\mod \rightarrow #2\!-\!\!\!\!\!\mod} % 
%\newcommand{\SP}{Snoopy-Peanutzovic}
\newcommand{\SP}{Burau--Rittenberg}
\newcommand{\Diff}{Dif\!f}  %% diffeo
\newcommand{\FF}{{\mathsf F}} % hook for functor
\newcommand{\FFF}{{\mathsf f}} % hook for generic functor

\newcommand\nn{n}
\newcommand\nno{{n-1}}

\newcommand\PB[1]{PB_{#1}}	% pure braid groups

\newcommand\PLB[1]{PLB_{#1}}	% pure loop braid groups

\newcommand\rr[1]{\rho_{\hspace{-0.3ex}#1}^{\null}}	%generators of permutations with well behaved spacing
\newcommand{\pp}{p}
\newcommand\rrp[1]{\pp_{\hspace{-0.3ex}#1}^{}}	%generators of permutations with well behaved spacing
\newcommand\rrb[1]{\rhob_{\hspace{-0.3ex}#1}^{\null}}	%hook for generalised Burau
\newcommand\rrq[2]{\rho_{\hspace{-0.3ex}#1}^{#2}}	%square of generators of permutations
\newcommand\rinv[1]{\rrq{#1}{-1}}	%inverse of generators of permutations
\newcommand\rrf[1]{\rrq{#1}{-}}	%formal inverse of generators of permutations

\newcommand\sig[1]{\sigma_{\hspace{-0.3ex}#1}^{\null}} % sigma generators with well behaved spacing
\newcommand\sigg[2]{\sigma_{\hspace{-0.3ex}#1}^{#2}}	%square of generators of braids
\newcommand\siginv[1]{\sigg{#1}{-1}}	%inverse of generators of braids
\newcommand\sigf[1]{\sigg{#1}{-}}	%formal inverse of generators of braids

\newcommand\WB[1]{WB_{#1}}	%welded braid group
\newcommand\WP[1]{WP_{#1}}	%pure welded braid group

\newcommand{\R}{{\mathfrak R}}  %% the extra relations for LH
\newcommand{\Q}{{\mathfrak Q}}  %% the relations for LB
\newcommand{\A}{{\mathfrak A}}  %% the relations for B

\newcommand{\Scat}{{\mathsf S}} %% a cat hook
\newcommand{\rrr}{r} %% a representation hook
\newcommand{\MMM}{{\mathcal M}}  % pascal matrix

\newcommand{\Mot}{{\mathcal Mo}}  %% motion gp
\newcommand{\un}[1]{\underline{#1}} 

\newcommand{\e}{{\mathbf e}}
\newcommand{\ket}[1]{ | #1 \rangle } 
%\newcommand{\Ccat}{{\mathsf C}}
\newcommand{\Ccat}{{\mathbf C}}


\newcommand{\rb}[2]{\raisebox{#1pt}{#2}}
\newcommand{\BOX}{\rb{-4}{\includegraphics[width=1cm]{xfig/cup1.eps}}}
\newcommand{\DUAL}{\rb{-4}{\includegraphics[width=1cm]{xfig/cap1.eps}}}
\newcommand{\ud}{{\mathsf u}}
\newcommand{\Tcat}{{\mathsf T}}
\newcommand{\ttt}{\tau}
\newcommand{\U}{{\mathsf U}}
\newcommand{\G}{{\mathsf G}}
\newcommand{\GU}{\G_{\U}}
\newcommand{\ups}{\Upsilon}
\newcommand{\FCAT}{(\Bcat,\Mat^{3c}_{k})}
\newcommand{\ob}{\underline{ob}}
\newcommand{\mate}{{\tiny \mat{cc} a&b\\ c&d\tam}}
\newcommand{\HH}{{\mathcal H}}
\newcommand{\integ}{{natural}}
\newcommand{\Or}[2]{{#1}_{|_{{#2}}}}  %% two constraint eqs for one!
\newcommand{\bc}{(b|c)}
\newcommand{\modelss}{\models^{\!\!\!\!\!\circ}} 
\newcommand{\gaml}{\gamma^l} 
\newcommand{\gamr}{\gamma^r} 


